SUOD: Accelerating Large-Scale Unsupervised Heterogeneous Outlier Detection

Outlier detection (OD) is a key machine learning (ML) task for identifying abnormal objects from general samples with numerous high-stake applications including fraud detection and intrusion detection. Due to the lack of ground truth labels, practitioners often have to build a large number of unsupervised, heterogeneous models (i.e., different algorithms with varying hyperparameters) for further combination and analysis, rather than relying on a single model. How to accelerate the training and scoring on new-coming samples by outlyingness (referred as prediction throughout the paper) with a large number of unsupervised, heterogeneous OD models? In this study, we propose a modular acceleration system, called SUOD, to address it. The proposed system focuses on three complementary acceleration aspects (data reduction for high-dimensional data, approximation for costly models, and taskload imbalance optimization for distributed environment), while maintaining performance accuracy. Extensive experiments on more than 20 benchmark datasets demonstrate SUOD's effectiveness in heterogeneous OD acceleration, along with a real-world deployment case on fraudulent claim analysis at IQVIA, a leading healthcare firm. We open-source SUOD for reproducibility and accessibility.

==> author_list.tex <==
\author{Yue Zhao}
\email{zhaoy@cmu.edu}
\affiliation{%
    \institution{Carnegie Mellon University}
}

\author{Xiyang Hu}
\email{xiyanghu@cmu.edu}
\affiliation{%
    \institution{Carnegie Mellon University}
}

\author{Cheng Cheng}
\email{ccheng2@andrew.cmu.edu}
\affiliation{%
    \institution{Carnegie Mellon University}
}

\author{Cong Wang}
\email{wangcong@gsm.pku.edu.cn}
% \email{wangc3.14@sem.tsinghua.edu.cn}
\affiliation{%
    % \institution{Tsinghua University}
    \institution{Peking University}
}

\author{Changlin Wan}
\email{wan82@purdue.edu}
\affiliation{%
    % \institution{Tsinghua University}
    \institution{Purdue University}
}

\author{Wen Wang}
\email{wenw3@andrew.cmu.edu}
\affiliation{%
    \institution{Carnegie Mellon University}
}

Jianing Yang\\
%   Machine Learning Department\\
  Carnegie Mellon University\\
  \texttt{jianing3@cs.cmu.edu} \\

Haoping Bai\\
%   Andrew ID: \texttt{HAOPINGB}\\
%   Machine Learning Department\\
  Carnegie Mellon University\\
  \texttt{haopingb@andrew.cmu.edu}\\

\author{Zheng Li}
\email{winston@arimadata.com}
\affiliation{%
    % \institution{Tsinghua University}
    \institution{Arima Inc., Canada}
}

\author{Cao Xiao}
\email{cao.xiao@iqvia.com}
\affiliation{%
    \institution{Analytics Center of Excellence, IQVIA}
}

\author{Yunlong Wang}
\email{yunlong.wang@iqvia.com}
\affiliation{%
    \institution{Department of Advanced Analytic, IQVIA}
}

\author{Zhi Qiao}
\email{zhi.qiao@iqvia.com}
\affiliation{%
    \institution{Analytics Center of Excellence, IQVIA}
}

\author{Jimeng Sun}
\email{jimeng@illinois.edu}
\affiliation{%
    % \institution{Univ. of Illinois Urbana-Champaign}
    \institution{University of Illinois at Urbana-Champaign}
    % \institution{UIUC}
}

\author{Leman Akoglu}
\email{lakoglu@andrew.cmu.edu}
\affiliation{%
    \institution{Carnegie Mellon University}
}

==> tables/algo_complexity.tex <==
% \yz{Table \ref{table:model_complexity} is added below; to be complete. However, it highly depends on implementation and optimization.} 

% \begin{table}%[ht]
% \centering
% 	\caption{Time complexity across select outlier detector; \textcolor{red}{time complexity for the same algorithm varies in different papers}} % title of Table
% 	\begin{tabular}{l l |  r  r } % centered columns (4 columns)
% 		\hline %inserts double horizontal lines
% 		\textbf{Method} & \textbf{Type} & \textbf{Training} & \textbf{Scoring}\\
% 		\hline
% 		$k$NN & slow  &  $\mathcal{O}(n^2d)$  & $\mathcal{O}(n)$ \\
% 		LOF   & slow  &  $\mathcal{O}(n^2)$   & $\mathcal{O}(n^2)$ \\
% 		LOCI  & slow  &  $\mathcal{O}(n^3)$   & $\mathcal{O}(nlog(n))$ \\
% 		TBC   & TBC   &  TBC   & TBC   \\
% 		\hline
% 	\end{tabular}
% 	\label{table:model_complexity} % is used to refer this table in the text
% \end{table}

==> tables/results_projection.tex <==
\begin{table*}[htb]
    \caption{Comparison of various projection methods on different outlier detectors and datasets.
    Each column corresponds to an evaluation metric; the best performing method is indicated in \textbf{bold}.}
    \footnotesize
    \label{table:projection_comparison}
    \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{ABOD on \textbf{MNIST}}\label{subtab:abod_mnist}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	        &	12.89	&	0.80	&	\textbf{0.39}	\\
                PCA	                &	8.93	&	\textbf{0.81}	&	0.37	\\
                RS	                &	\textbf{8.27}	&	0.74	&	0.32	\\
                \textit{basic}	    &	8.94	&	0.80	&	0.38	\\
                \textit{discrete}	&	8.86	&	0.80	&	\textbf{0.39}	\\
                \textit{circulant}	&	9.33	&	0.80	&	0.38	\\
                \textit{toeplitz}	&	8.96	&	0.80	&	0.38	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}%
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{ABOD on \textbf{Satellite}}\label{subtab:abod_satellite}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	4.03	&	0.59	&	0.41	\\
                PCA	&	\textbf{3.01}	&	0.62	&	0.44	\\
                RS &	3.53	&	0.63	&	0.44	\\
                \textit{basic}	&	3.10	&	0.64	&	0.45	\\
                \textit{discrete}	&	3.12	&	0.65	&	0.46	\\
                \textit{circulant}	&	3.14	&	\textbf{0.66}	&	\textbf{0.48}	\\
                \textit{toeplitz}	&	3.14	&	\textbf{0.66}	&	0.47	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{ABOD on \textbf{Satimage-2}}\label{subtab:abod_satimage}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	3.68	&	0.85	&	0.28	\\
                PCA	&	\textbf{2.70}	&	0.88	&	0.30	\\
                RS &	3.20	&	0.89	&	0.28	\\
                \textit{basic}	&	2.78	&	0.91	&	0.29	\\
                \textit{discrete}	&	2.79	&	0.91	&	\textbf{0.31}	\\
                \textit{circulant}	&	2.85	&	0.91	&	0.29	\\
                \textit{toeplitz}	&	2.83	&	\textbf{0.92}	&	0.30	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{ABOD on \textbf{Cardio}}\label{subtab:abod_cardio}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.98	&	0.59	&	0.25	\\
                PCA	&	\textbf{0.82}	&	0.59	&	0.26	\\
                RS &	0.92	&	\textbf{0.63}	&	\textbf{0.29}	\\
                \textit{basic}	&	0.83	&	0.62	&	0.28	\\
                \textit{discrete}	&	\textbf{0.82}	&	0.62	&	0.28	\\
                \textit{circulant}	&	0.83	&	0.62	&	0.27	\\
                \textit{toeplitz}	&	0.83	&	0.62	&	0.28	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
    
    \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{LOF on \textbf{MNIST}}\label{subtab:lof_mnist}
        
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	7.64	&	0.68	&	0.29	\\
                PCA	&	4.92	&	0.67	&	0.27	\\
                RS &	\textbf{3.65}	&	0.63	&	0.23	\\
                \textit{basic}	&	4.87	&	0.70	&	0.31	\\
                \textit{discrete}	&	5.21	&	0.70	&	\textbf{0.32}	\\
                \textit{circulant}	&	5.06	&	0.69	&	0.31	\\
                \textit{toeplitz}	&	4.97	&	\textbf{0.71}	&	0.31	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}%
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{LOF on \textbf{Satellite}}\label{subtab:lof_satellite}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.82	&	\textbf{0.55}	&	0.37	\\
                PCA	&	\textbf{0.23}	&	0.54	&	0.36	\\
                RS &	0.39	&	0.54	&	0.37	\\
                \textit{basic}	&	0.31	&	0.54	&	0.37	\\
                \textit{discrete}	&	0.32	&	0.54	&	0.37	\\
                \textit{circulant}	&	0.39	&	\textbf{0.55}	&	\textbf{0.38}	\\
                \textit{toeplitz}	&	0.37	&	0.54	&	0.37	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{LOF on \textbf{Satimage-2}}\label{subtab:lof_satimage}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.79	&	0.54	&	0.07	\\
                PCA	&	\textbf{0.20}	&	0.52	&	0.04	\\
                RS &	0.37	&	0.53	&	0.08	\\
                \textit{basic}	&	0.29	&	0.52	&	0.08	\\
                \textit{discrete}	&	0.30	&	0.53	&	0.07	\\
                \textit{circulant}	&	0.43	&	\textbf{0.59}	&	\textbf{0.11}	\\
                \textit{toeplitz}	&	0.32	&	0.54	&	0.09	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{LOF on \textbf{Cardio}}\label{subtab:lof_cardio}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.08	&	0.55	&	0.17	\\
                PCA	&	\textbf{0.04}	&	0.56	&	0.19	\\
                RS &	\textbf{0.04}	&	0.57	&	0.15	\\
                \textit{basic}	&	\textbf{0.04}	&	\textbf{0.60}	&	0.20	\\
                \textit{discrete}	&	\textbf{0.04}	&	0.59	&	0.19	\\
                \textit{circulant}	&	\textbf{0.04}	&	0.59	&	0.20	\\
                \textit{toeplitz}	&	\textbf{0.04}	&	\textbf{0.60}	&	\textbf{0.21}	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
    
 \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{$k$NN on \textbf{MNIST}}\label{subtab:knn_mnist}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	7.13	&	\textbf{0.84}	&	\textbf{0.42}	\\
                PCA	&	    3.92	&	\textbf{0.84}	&	0.40	\\
                RS &	\textbf{3.33}	&	0.77	&	0.34	\\
                \textit{basic}	&	4.17	&	\textbf{0.84}	&	\textbf{0.42}	\\
                \textit{discrete}	&	4.11	&	\textbf{0.84}	&	0.41	\\
                \textit{circulant}	&	4.13	&	\textbf{0.84}	&	0.41	\\
                \textit{toeplitz}	&	4.11	&	\textbf{0.84}	&	\textbf{0.42}	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}%
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{$k$NN on \textbf{Satellite}}\label{subtab:knn_satellite}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.71	&	0.67	&	0.49	\\
                PCA	&	\textbf{0.18}	&	0.67	&	0.50	\\
                RS &	0.31	&	0.68	&	0.49	\\
                \textit{basic}	&	0.24	&	0.68	&	0.49	\\
                \textit{discrete}	&	0.25	&	0.69	&	0.50	\\
                \textit{circulant}	&	0.33	&	\textbf{0.70}	&	0.50	\\
                \textit{toeplitz}	&	0.30	&	\textbf{0.70}	&	\textbf{0.51}	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{$k$NN on \textbf{Satimage-2}}\label{subtab:knn_satimage}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.68	&	0.94	&	\textbf{0.39}	\\
                PCA	&	\textbf{0.15}	&	0.94	&	\textbf{0.39}	\\
                RS &	0.29	&	0.94	&	0.38	\\
                \textit{basic}	&	0.23	&	0.94	&	0.38	\\
                \textit{discrete}	&	0.20	&	0.95	&	0.37	\\
                \textit{circulant}	&	0.36	&	\textbf{0.96}	&	0.37	\\
                \textit{toeplitz}	&	0.25	&	\textbf{0.96}	&	\textbf{0.39}	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
   \begin{subtable}[t]{.23\textwidth}
        \centering
        \caption{$k$NN on \textbf{Cardio}}\label{subtab:knn_cardio}
            \begin{tabular}{@{\extracolsep{1pt}}l  r r r r }
                \toprule
                \textbf{Method}	&	\textbf{Time}	&	\textbf{ROC}		&   \textbf{P@N}     \\
                \midrule 
                original	&	0.09	&	0.71	&	0.34	\\
                PCA	&	\textbf{0.03}	&	0.73	&	0.34	\\
                RS &	\textbf{0.03}	&	0.69	&	\textbf{0.38}	\\
                \textit{basic}	&	\textbf{0.03}	&	\textbf{0.74}	&	0.35	\\
                \textit{discrete}	&	\textbf{0.03}	&	\textbf{0.74}	&	0.37	\\
                \textit{circulant}	&	\textbf{0.03}	&	\textbf{0.74}	&	0.34	\\
                \textit{toeplitz}	&	\textbf{0.03}	&	0.73	&	0.35	\\
                \bottomrule \\
            \end{tabular}
    \end{subtable}
\end{table*}
